The House That Knows You: User Authentication Based on IoT Data

Home-based Internet of Things (IoT) devices have gained in popularity and many households have become 'smart' by using devices such as smart sensors, locks, and voice-based assistants. Traditional authentication methods such as passwords, biometrics or multi-factor (using SMS or email) are either not applicable in the smart home setting, or they are inconvenient as they break the natural flow of interaction with these devices. Voice-based biometrics are limited due to safety and privacy concerns. Given the limitations of existing authentication techniques, we explore new opportunities for user authentication in smart home environments. Specifically, we design a novel authentication method based on behavioral features extracted from user interactions with IoT devices. We perform an IRB-approved user study in the IoT lab at our university over a period of three weeks. We collect network traffic from multiple users interacting with 15 IoT devices in our lab and extract a large number of features to capture user activity. We experiment with multiple classification algorithms and also design an ensemble classifier with two models using disjoint set of features. We demonstrate that our ensemble model can classify five users with 0.97 accuracy. The behavioral authentication modules could help address the new challenges emerging with smart home ecosystems and they open up the possibility of creating flexible policies for authorization and access control.

==> features.tex <==
\subsection{Feature Representation}


\begin{table*}[h]
	\begin{center}
		\begin{tabular}{|p{0.20\textwidth}|p{0.15\textwidth}|p{0.65\textwidth}|}
			\hline
			{\bf Feature} & {\bf Type} & {\bf Description} \\
			\hline
			Device Name & Categorical & Name of the smart device \\
			\hline
			Timedelta & Integer & The timestamp of the packet in seconds within the window\\
			\hline
			Packet Length & Integer & Size of the packet in bytes\\
			\hline
			Domain & Categorical & Domain name of the server, if available\\
			\hline
			Direction & Categorical & Direction of the packet (outgoing/incoming)\\
			\hline
			Protocol & Categorical & Transport protocol of the packet (TCP/UDP)\\
			\hline
			Destination Port & Categorical & Port number of the destination address\\
			\hline
			Source Port & Categorical & Port number of the source address\\
			\hline
		\end{tabular}
	\end{center}
	\caption{{\bf Packet Level Features:} These features are generated for each packet in a given time window. }
	\label{table_packetlevel}
\end{table*}


\begin{table*}[]
	\begin{tabular}{|c|c|c|}
		\hline
		\textbf{Feature Category} & \textbf{Operations}                     & \textbf{Description}                             \\ \hline
		Incoming packet lengths   & count, sum, min, max, std, mean, median & Extract statistics on incoming packet lengths    \\ \hline
		Outgoing packet lengths   & count, sum, min, max, std, mean, median & Extract statistics on outgoing packet lengths    \\ \hline
		Protocols                 & count                                   & Packet counts for each protocol (TCP, UDP, ICMP) \\ \hline
		Domains                   & distinct                                & Distinct domain count                            \\ \hline
		Inter-event times         & count, sum, min, max, std, mean, median & Extract statistics on inter-packet time array    \\ \hline
	\end{tabular}
	\caption{{\bf Aggregated packet statistics features:} For each aggregation window, the feature vector consists of these values. The three feature representations are (1) Generating these features except inter-event times for each device, (2) Generating these features with inter-event times for each device, (3) Generating these features for each device and domain.}
	\label{table_packet_stats}
\end{table*}


We collected network data in pcap files on our monitoring server. The user study provided us the timings of each session for users to be able to label the respective data with the user id. We use sliding time window parameter (T) to split each session into multiple data samples labeled with the user of the session. The window slides by 60 seconds between the samples. For example, for T=10 minutes and session start time S, the first sample interval is from S to S+10 minutes while the second sample is from S+1 to S+11. After each sample time intervals and labels are defined, first step of processing was to fetch relevant information from each packet to strip out irrelevant information (e.g. the payload).

\subsubsection{Packet Attributes}

We parse the pcap traces and built a database that contains the packet header fields as the traffic is mostly encrypted and we want to build our system that relies on patterns over time as opposed to deep packet inspection which might put user privacy at risk. We further include the DNS queries in our database as this would make it easier for us to find the domain name of the external IP addresses that are communicated.
From the packet headers, we extract the timestamp, source IP, destination IP, protocol, destination port, source port, and packet length information. Since external IP addresses that these devices communicate for the same service can change over time, we decide to use the domain names instead of the IP addresses. We look for the DNS request messages in the dataset to find the domain names of the IP addresses. The domain name information might not always available due to the hard-coding of the IP address, meaning DNS request has not been made, or a request has been made a long time ago that our captured data does not contain it. We defined another domain name 'none' to fill in those cases. We could rely on SNI information in the TLS handshake. However, some devices do not use TLS and even if they do, they might not be using SNI to reveal the domain names. The internal IP, which is the IP address of the devices can also change over time and does not contain relevant information. Instead, we defined a field 'direction' to indicate if the packet is outgoing (from device to external server) or incoming (from external server to device). The absolute timestamp information is not relevant as we do not model the user behavior based on time of day or day of week. We instead use relative time in seconds within the time period makes more sense as we keep the sequential information and inter-packet times. Finally, we add the device name information to each packet since we know the MAC addresses of each device and each packet contains the MAC address.

Using these defined packet fields to train machine learning models is not scalable in terms of both training process as it will be more difficult to learn the behavior from a big feature space and small number of samples and real time testing process as it would require the system to collect all network traffic represent each packet individually. Therefore, some form of aggregation is necessary.

\begin{figure*}[ht]
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/heatmap_sum.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/heatmap_count.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/heatmap_average.pdf}
		
	\end{minipage}
	\captionsetup{justification=centering,margin=2cm}
	\caption{High level device usage statistics from the user study. \\Total bytes sum, packet count and average bytes size over packets are plotted from left to right.}
	\label{fig:figure_deviceusage}
\end{figure*}


\begin{figure*}[ht]
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/heatmap_sumDomains.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/heatmap_countDomains.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/heatmap_averageDomains.pdf}
		
	\end{minipage}
	\captionsetup{justification=centering,margin=2cm}
	\caption{High level domain usage statistics from the user study. \\Total bytes sum, packet count and average bytes size over packets are plotted from left to right.}
	\label{fig:figure_domainusage}
\end{figure*}


\begin{figure*}[ht]
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user6_3selecteddevices.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user6_8selecteddevices.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user6_33selecteddevices.pdf}
		
	\end{minipage}
	\captionsetup{justification=centering,margin=2cm}
	\caption{Usage of some devices for user 6 in 3 of the sessions}
	\label{fig:figure_user6_sessions}
\end{figure*}

\begin{figure*}[ht]
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user8_17selecteddevices.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user8_46selecteddevices.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user8_55selecteddevices.pdf}
		
	\end{minipage}
	\captionsetup{justification=centering,margin=2cm}
	\caption{Usage of some devices for user 8 in 3 of the sessions}
	\label{fig:figure_user8_sessions}
\end{figure*}

\begin{figure*}[ht]
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user10_26selecteddevices.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user10_49selecteddevices.pdf}
		
	\end{minipage}
	\hspace{0.5cm}
	\begin{minipage}[b]{0.3\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/user10_54selecteddevices.pdf}
		
	\end{minipage}
	\captionsetup{justification=centering,margin=2cm}
	\caption{Usage of some devices for user 10 in 3 of the sessions}
	\label{fig:figure_user10_sessions}
\end{figure*}

\subsubsection{Data Aggregation}

We explore different representations that would be suitable for our task of user classification. First observation we have is that different user actions lead to different user profiles and the actions that involve a smart device could be detectable by the respective device. This led us to think of device based aggregation methods as we know the device information for in the network traffic. We analyzed the data we collected to compare how different users were in terms of the devices they used. In the heatmaps in figure \ref{fig:figure_deviceusage}, you can see for some devices such as Amazon Echospot and Google Home, the amount of data exchanged varies by user. On the other hand, it becomes obvious that some smart devices are either not being used by the users or are not very active on the network. The patterns can be seen for total exchanged data amount as well as total packet counts and they look to be correlated.

We observed in the data that some devices, such as Amazon Echo Dot, communicated with multiple different domains depending on what the user asks. E.g. if the user listens to music, data comes from Spotify domain. In order to capture different user actions in a more fine grained way, we decided to include domain based aggregation to our feature set. We noticed that there are many similar names from the same second level domain, and they are used for the same tasks. Therefore, instead of using the full domain name, we group the data based on second-level domain names.
The high-level domain usage statistics is shown in figure \ref{fig:figure_domainusage}. It includes the second-level domains that has more than 10000 packets and their usage patterns per user. We observe the different usage patterns that suggests that modeling the users and separating them can be possible using domain based feature aggregation.

The first features we decided to define were the exchanged data size in both directions for each device and each domain. Having separate features for the direction of the data makes sense as it would be an important factor for personal voice assistants (e.g. Amazon Echo Dot, Google Home) since they transmit the voice data to the cloud servers for processing. The first set of aggregated features included the amount of data exchanged for each device for both directions. This simple aggregation method results in a single array summing packet lengths and counts. However, it loses the information about the timing and fine grained structure of the actions. For example, the user might have a pattern of using Amazon Echo Dot with 5 minute intervals, which would not be apparent in our feature vector. We decided to include information about inter-event timings for each domain and device. More specifically, we extract sum, count, mean, median, standard deviation, min and max values from the inter-event array where each element represents the time between the two consecutive packets belonging to the device or domain. We further decided to include the same statistical values for both incoming and outgoing packet lengths instead of having a single sum value to further include finer grained information. Furthermore, protocol usage information that includes packet sounds for TCP, ICMP, and UDP is also added to capture protocol usage differences for each device and domain. For each device, the distinct domain names contacted feature is also added. The list of features that we refined could be seen in table \ref{table_packet_stats}.


